A comparison of smooth basis constructions for isogeometric analysis

In order to perform isogeometric analysis with increased smoothness on complex domains, trimming, variational coupling or unstructured spline methods can be used. The latter two classes of methods require a multi-patch segmentation of the domain, and provide continuous bases along patch interfaces. In the context of shell modeling, variational methods are widely used, whereas the application of unstructured spline methods on shell problems is rather scarce. In this paper, we therefore provide a qualitative and a quantitative comparison of a selection of unstructured spline constructions, in particular the D-Patch, Almost-$C^1$, Analysis-Suitable $G^1$ and the Approximate $C^1$ constructions. Using this comparison, we aim to provide insight into the selection of methods for practical problems, as well as directions for future research. In the qualitative comparison, the properties of each method are evaluated and compared. In the quantitative comparison, a selection of numerical examples is used to highlight different advantages and disadvantages of each method. In the latter, comparison with weak coupling methods such as Nitsche's method or penalty methods is made as well. In brief, it is concluded that the Approximate $C^1$ and Analysis-Suitable $G^1$ converge optimally in the analysis of a bi-harmonic problem, without the need of special refinement procedures. Furthermore, these methods provide accurate stress fields. On the other hand, the Almost-$C^1$ and D-Patch provide relatively easy construction on complex geometries. The Almost-$C^1$ method does not have limitations on the valence of boundary vertices, unlike the D-Patch, but is only applicable to biquadratic local bases. Following from these conclusions, future research directions are proposed, for example towards making the Approximate $C^1$ and Analysis-Suitable $G^1$ applicable to more complex geometries.

==> Sections/Preliminaries.tex <==
\PW{Need a review and check if something is missing for notation or not explained carefully. If you want to change the notation or extend some explanation, feel free to do this :)}


In this section we introduce briefly the overview of B-spline and their spaces as well as their notations. In ???, a more detailed discussion can be found. For constructing the geometry as well as for the discrete space, we use spline functions, namely the B-splines. As usual, these basis functions can be constructed with the Cox-de Boor recursion and span the one-dimensional spline space denoted by
\begin{equation}
\mathcal{S} (p, r, h),
\end{equation}
where $p$ is the polynomial degree, $r$ the regularity and $h$ the mesh-size. For simplicity, we assume that the spline basis functions are uniformly constructed with the same multiplicity for each inner knots. It follows that the spline space consists of functions which are $C^r$-continuous on the parameter domain.
In two-dimensional case, the spline space is defined by the tensor-product structure as following
\begin{equation}
\vb{\mathcal{S}} (\vb p, \vb r, \vb h) = \mathcal{S} (p, r, h) \otimes \mathcal{S} (p, r, h),
\end{equation}
where $\vb p = (p,p)$, $\vb r = (r,r)$ and $\vb h = (h,h)$. Again, we assume throughout in this paper that the polynomial degree, regularity and mesh sizes are the same for each spline space.
Furthermore, let $\Omega$ be a multi-patch segmentation consisting of non-overlapping patches $\Omega^{(k)}$, i.e., we have
\[
\Omega = \bigcup_k \Omega^{(k)}
\]
with $\Omega^{(k)} \cap \Omega^{(l)} = \empty$ for all $k \neq l$. Then, we introduce for each patch $\Omega^{(k)}$ the geometry mapping $\vb{F}^{(k)}$ with
\[
\vb{F}^{(k)} \, : \, \hat{\Omega} = [0,1]^2 \to \overline{\Omega^{(k)}}.
\]
We assume that each geometry mapping is regular and does not self-overlap.
Finally, we can present the definition of the isogeometric multi-patch spaces which consist of isogeometric functions $\varphi : \Omega \to \mathcal{R}$ with
\[
\varphi \circ \vb{F}^{(k)} \in \vb{S}^{(k)}.
\]
We assume that the patches meet $C^0$ at the interfaces in order to have the $C^0$-conformity at the interfaces. Then we introduce the $C^0$ space, namely the $C^0$ isogeometric multi-patch space. Follow ???, this space is given as
\[
\mathcal{X}_h = \{ \varphi \in C^0 (\Omega) \text{ such that } w^{(k)} = \varphi \circ \vb{F}^{(k)} \in \vb{S}^{(k)} \; \forall k \}.
\]
Since our aim of the paper is to solve fourth-order PDEs or in general, to construct spline basis functions which are or behave like $C^1$ spline basis functions, we introduce the space
\[
\mathcal{V} = \{ \varphi \in H^2 (\Omega) \},
\]
where $H^2$ is the standard Sobolev space over $\Omega$.
\PW{From here on, it gets a bit complicated. We need the patch-wise inner-product. Maybe we can avoid it. I don't know...}

%\begin{itemize}
%    \item Spline space
%    \item Multi-patch geometry
%    \item $C^0$ spline space
%    \item $C^1$ spline space
%\end{itemize}

